Channel Cycle Time: A New Measure of Short-term Fairness

This paper puts forth a new metric, dubbed channel cycle time (CCT), to measure the short-term fairness of communication networks. CCT characterizes the average duration between two consecutive successful transmissions of a user, during which all other users successfully accessed the channel at least once. In contrast to existing short-term fairness measures, CCT provides more comprehensive insight into the transient dynamics of communication networks, with a particular focus on users' delays and jitter. To validate the efficacy of our approach, we analytically characterize the CCTs for two classical communication protocols: slotted Aloha and CSMA/CA. The analysis demonstrates that CSMA/CA exhibits superior short-term fairness over slotted Aloha. Beyond its role as a measurement metric, CCT has broader implications as a guiding principle for the design of future communication networks by emphasizing factors like fairness, delay, and jitter in short-term behaviors.

==> meeting.tex <==
多址接入协议问题是一个经典问题，因为是为了解决interfere，为了衡量其性能提出了各种指标：
saturated traffic -> unsaturated traffic

1. throughput - long-term metric, 单位时间内网络传输包的个数
2. delay - pdf
3. jitter
4. collision rate
5. fairness ()

多址接入问题
fairness
short-term fairness
提出了...,重点在fairness，顺便也能反映throughput


几个问题：

1. CSMA的P0：实际上并非不随CW改变
number of inter-transmission的paper里认为不变，是因为把各个CW近似为连续的，这样碰撞概率很小。因此可以认为，如果碰撞概率很小，那么P0就近似不变。
仿真结果表明，CW>=32后，P0变化很小（1.47-1.49）。但CW较小时，P0会更小（1.40左右）。
因此仿真CSMA时，最小的CW值设为32。这样channel cycle time随着CW单调增，见Fig 6，无法取到理论的最小值。
（理论上会先下降再上升，见(16)式，CW>32时已经超过了分界点，因此一直上升。
此外，如上所述，实际上CW较小时P0也较小，因此仿真结果显示即使CW较小，也是随CW单调增，没有下降的情况）

2. slotted ALOHA只有理论结果，没有仿真。
因此在比较时，见Fig 7，均使用的理论值。

3.cite的paper都比较老（最新的是2014）





1. 资源分配过程中fairness的重要性
2. fairness分为long和short,long有哪些measure，short term的区别是什么？为何值得关注？
3. short term受到关注少，已经有的measure是什么？缺点是？
4. 本文的主要贡献：1)提出...,有何优势？2)分析


改：
1. 资源分配过程中fairness的重要性
2. fairness的measure。分为long和short，区别是什么？short为何值得关注？
4. short term受到关注少，如何measure？缺点是？
5. 本文的主要贡献：1)提出...,有何优势？2)分析


1. fig6:
删掉basic mode 和 rtc/cts
analytical/numerical results and simulation results
结论：
1) 分析和仿真一致
2) slotted最差
3) CSMA/CA和TDMA的gap
2. 比较basic和rts/cts,随着包长

3. 加一张table写参数
TDMA, slotted ALOHA, CSMA/CA

